A Bi-Criteria FPTAS for Scheduling with Memory Constraints on Graph with Bounded Tree-width

In this paper we study a scheduling problem arising from executing numerical simulations on HPC architectures. With a constant number of parallel machines, the objective is to minimize the makespan under memory constraints for the machines. Those constraints come from a neighborhood graph G for the jobs. Motivated by a previous result on graphs G with bounded path-width, our focus is on the case when the neighborhood graph G has bounded tree-width. Our result is a bi-criteria fully polynomial time approximation algorithm based on a dynamic programming algorithm. It allows to find a solution within a factor of 1 + epsilon of the optimal makespan, where the memory capacity of the machines may be exceeded by a factor at most 1 + epsilon. This result relies on the use of a nice tree decomposition of G and its traversal in a specific way which may be useful on its own. The case of unrelated machines is also tractable with minor modifications.

==> img/figlemma2.tex <==
\begin{tikzpicture}[
    white/.style={circle, draw=black, fill=white,text centered, anchor=north, text=black},
    red/.style={circle, draw=black, fill=red!70!white,
        text centered, anchor=north, text=black},
    yellow/.style={circle, draw=red, fill=yellow!90!black,
        text centered, anchor=north, text=black},
    void/.style={circle, draw=none},
    level distance=0.5cm, growth parent anchor=south, scale=0.7, every node/.style={transform shape}
]
\node (Root) [red] {$174$} [-, sibling distance=2cm] 
    child{ [sibling distance=1cm]
        node (100) [yellow] {$100$}
	 	child{ 
        			node (100lf) [void] {} edge from parent[draw=none]
		 	child{ 
        				node (100l) [void] {} edge from parent[draw=none]
			}   
		}   
	 	child{
        			node (100rf) [void] {} edge from parent[draw=none]
		 	child{ 
        				node (100r) [void] {} edge from parent[draw=none]
			}   
		}   
    }   
    child{ [sibling distance=1.4cm]
        node (173) [white] {$173$}
 	child{  [sibling distance=2.4cm]
        		node (172) [red] {$172$}
	 	child{  [sibling distance=1cm]
        			node (140) [yellow] {$140$}
	 		child{ 
        				node (140lf) [void] {} edge from parent[draw=none]
		 		child{ 
        					node (140l) [void] {} edge from parent[draw=none]
				}   
			}   
		 	child{
        				node (140rf) [void] {} edge from parent[draw=none]
		 		child{ 
        					node (140r) [void] {} edge from parent[draw=none]
				}   
			}   
		}   
	 	child{  [sibling distance=2cm]
        			node (171) [red] {$171$}
	 		child{  [sibling distance=1cm]
        				node (160) [yellow] {$160$}
		 		child{ 
        					node (160lf) [void] {} edge from parent[draw=none]
		 			child{ 
        						node (160l) [void] {} edge from parent[draw=none]
					}   
				}   
		 		child{
        					node (160rf) [void] {} edge from parent[draw=none]
		 			child{ 
        						node (160r) [void] {} edge from parent[draw=none]
					}   
				}   
			}   
	 		child{  [sibling distance=1.4cm]
        				node (170) [white] {$170$}
		 		child{  [sibling distance=1.4cm]
        					node (169) [white] {$169$}
			 		child{  [sibling distance=2cm]
        						node (168) [red] {$168$}
				 		child{  [sibling distance=1cm]
        							node (165) [yellow] {$165$}
					 		child{  
        								node (165lf) [void] {} edge from parent[draw=none]
		 						child{ 
        									node (165l) [void] {} edge from parent[draw=none]
								}   
							}   
					 		child{
        								node (165rf) [void] {} edge from parent[draw=none]
		 						child{ 
        									node (165r) [void] {} edge from parent[draw=none]
								}   
							}   
						}   
				 		child{
        							node (167) [white] {$167$}
				 			child{
        								node (166) [yellow] {$166$}
							}   
						}   
					}   
			 		child{
        						node (v3) [void] {} edge from parent[draw=none]
					}   
				}   
		 		child{
        					node (v2) [void] {} edge from parent[draw=none]
				}   
			}   
		}   
	}   
 	child{
        		node (v1) [void] {} edge from parent[draw=none]
	}   
    }   
;


\draw (100) -- (100l.center) -- (100r.center) -- (100);
\draw (140) -- (140l.center) -- (140r.center) -- (140);
\draw (160) -- (160l.center) -- (160r.center) -- (160);
\draw (165) -- (165l.center) -- (165r.center) -- (165);

\draw (165lf)++(-0.5,0) node{size $5$} ;
\draw (160lf)++(-0.5,0) node{size $20$} ;
\draw (140lf)++(-0.5,0) node{size $40$} ;
\draw (100lf)++(-0.65,0) node{size $100$} ;

\draw (Root)++(1,0) node{Root} ;
\draw (166)++(1.15,0) node{$L^{-1}(i)$} ;

\end{tikzpicture}


==> img/figlemma2part2.tex <==
\begin{tikzpicture}[
    white/.style={circle, draw=black, fill=white,text centered, anchor=north, text=black},
    red/.style={circle, draw=black, fill=red!70!white,
        text centered, anchor=north, text=black},
    yellow/.style={circle, draw=red, fill=yellow!90!black,
        text centered, anchor=north, text=black},
    void/.style={circle, draw=none},
    level distance=0.5cm, growth parent anchor=south, scale=0.7, every node/.style={transform shape}
]
\node (Root) [red] {$174$} [-, sibling distance=2.4cm] 
    child{ [sibling distance=1cm]
        node (100) [yellow] {$100$}
	 	child{ 
        			node (100lf) [void] {} edge from parent[draw=none]
		 	child{ 
        				node (100l) [void] {} edge from parent[draw=none]
			}   
		}   
	 	child{
        			node (100rf) [void] {} edge from parent[draw=none]
		 	child{ 
        				node (100r) [void] {} edge from parent[draw=none]
			}   
		}   
    }   
    child{ [sibling distance=2.2cm]
        node (172) [red] {$172$}
	 	child{ [sibling distance=1cm]
        			node (140) [yellow] {$140$} 
		 	child{  
        				node (140lf) [void] {} edge from parent[draw=none]
			 	child{ 
        					node (140l) [void] {} edge from parent[draw=none]
				}   
			}   
		 	child{
        				node (140rf) [void] {} edge from parent[draw=none]
		 		child{ 
        					node (140r) [void] {} edge from parent[draw=none]
				}   
			}   
		}   
	 	child{ [sibling distance=1.9cm] 
        			node (171) [red] {$171$}
		 	child{ [sibling distance=1cm]
        				node (160) [yellow] {$160$} 
			 	child{ 
        					node (160lf) [void] {} edge from parent[draw=none]
				 	child{ 
        						node (160l) [void] {} edge from parent[draw=none]
					}   
				}   
			 	child{
        					node (160rf) [void] {} edge from parent[draw=none]
		 			child{ 
        						node (160r) [void] {} edge from parent[draw=none]
					}   
				}   
			}   
		 	child{ [sibling distance=1.4cm] 
        				node (168) [red] {$168$} 
				 child{ [sibling distance=1cm]
        					node (165) [yellow] {$165$} 
				 	child{ 
        						node (165lf) [void] {} edge from parent[draw=none]
					 	child{ 
        							node (165l) [void] {} edge from parent[draw=none]
						}   
					}   
				 	child{
        						node (165rf) [void] {} edge from parent[draw=none]
		 				child{ 
        							node (165r) [void] {} edge from parent[draw=none]
						}   
					}   
				}   
			 	child{
        					node (166) [yellow] {$166$} 
				}   
			}   
		}   
    }   
;


\draw (100) -- (100l.center) -- (100r.center) -- (100);
\draw (140) -- (140l.center) -- (140r.center) -- (140);
\draw (160) -- (160l.center) -- (160r.center) -- (160);
\draw (165) -- (165l.center) -- (165r.center) -- (165);

\draw (100lf)++(-0.65,0) node{size $100$} ;
\draw (140lf)++(-0.65,0) node{size $40$} ;
\draw (160lf)++(-0.65,0) node{size $20$} ;
\draw (165lf)++(-0.65,0) node{size $5$} ;

\draw (Root)++(1,0) node{Root} ;
\draw (166)++(1.2,0) node{$L^{-1}(i)$} ;

\end{tikzpicture}

